Common Fate for Animated Transitions in Visualization

The Law of Common Fate from Gestalt psychology states that visual objects moving with the same velocity along parallel trajectories will be perceived by a human observer as grouped. However, the concept of common fate is much broader than mere velocity; in this paper we explore how common fate results from coordinated changes in luminance and size. We present results from a crowdsourced graphical perception study where we asked workers to make perceptual judgments on a series of trials involving four graphical objects under the influence of conflicting static and dynamic visual factors (position, size and luminance) used in conjunction. Our results yield the following rankings for visual grouping: motion > (dynamic luminance, size, luminance); dynamic size > (dynamic luminance, position); and dynamic luminance > size. We also conducted a follow-up experiment to evaluate the three dynamic visual factors in a more ecologically valid setting, using both a Gapminder-like animated scatterplot and a thematic map of election data. The results indicate that in practice the relative grouping strengths of these factors may depend on various parameters including the visualization characteristics and the underlying data. We discuss design implications for animated transitions in data visualization.

==> scraps.tex <==
% \jacob{Seems important to note that none of this is empirical!}
% \jacob{Talk about CHI 2018 paper on animated links}
% \jacob{re-iterate that the Generalized Common Fate studies were not applied to visualization}

% \subsection{Perception in Visualization}

% %\jacob{None of these seem directly applicable except as deep background - perhaps merge this with prior section?}

% Statisticians have long been interested in the perception of their charts.
% Examples of pioneering works on this topic include those of Eells~\cite{Eells1926}, Croxton~\cite{Croxton1932, Croxton1927}, and Peterson et al.~\cite{Peterson1954}.
% Recent studies have extended these works to interactive visualization.
% Representative examples include Haroz and Whitney's work on attention capacity~\cite{Haroz2012}, and Harrison et al.'s crowdsourced ranking of visualizations based on correlation~\cite{Harrison2014}.
% Heer and Bostock~\cite{Heer2010} have also demonstrated that graphical perception studies can be crowdsourced for a significantly lower cost than laboratory experiments with a negligible loss of precision.



%In the Gapminder condition, we also had three variables changing simultaneously, which may have compounded this distracting effect.
%It may have been less severe in the first experiment because of the lower number of simultaneously changing variables, and the lower number of visual objects, which enabled participants to track all 4 objects in parallel~\cite{Pylyshyn1988}.

% It is hence preferable, whenever possible, to have recourse to another visual variable for grouping.

% First, one should not use the same pair of visual variables for making groups perceptually emerge when a visualization is intended to treat several groups as equivalent, and, on the contrary, when a single group should be made more salient than any other group.

% .


% When it is important to enable conjunction search---\ie, when several groups should be identifiable at the time---a set of visual variables that have similar grouping strength when used together---\ie none of the variables dominates the others---should be preferred.
% For instance, imagine an animated transition between two scatterplots, where position only encodes data.
% During the transition, dots will inevitably move from their initial position to their final position.
% To make two groups emerge in such case (recall that \DP+\SP is not available), one can choose to use either the pair \SS/\SL for revealing two groups, or \DS/\DL.
% Other configurations, such as \SS/\DL, are more likely to create perceptual unbalance: \DL dominating \SS for grouping, the group encoded with \SS is prone to be unnoticed.


% Our empirical study on the effects of variable conjunction on perceptual grouping is an initial step towards more fleshed out design guidelines for dynamic information visualizations and animated transitions, and our follow-up study illustrates two possible ways Common Fate grouping can be applied in more realistic visualization scenarios.
% Here, we discuss situations where our results can guide design.

%\emph{Choice of visual variables.}



%The lack of a clear difference in Study 1, when \DP and \DS were compared in isolation, may also result from our difficulty in distinguishing between common-fate groups~\cite{Levinthal2011}.

%\jacob{Colin Ware Perception for Design pg. 181 - color and size are less separable than color/size and position. The iterative refinement strategies participants used when finding the closest point indicates that all three dynamic variables are fairly separable.}


%Our results also suggest several cases where two visual variables support conjunctive emphasis of two groups simultaneously.
% This is, for instance, the case for \DS and \SL; .
%, though users qualitative feedback suggests that \DL and \DS are more manageable when combined with each other than with \DP.


%% ---------------------------------------------------------------------
%% Followup Study
%% ---------------------------------------------------------------------
\section{Follow-up: Common Fate for Trend Visualization}
\label{sec:followup}

The main study in this paper was designed to maximize internal validity by carefully controlling and balancing each experimental factor, at the price of compromising ecological validity.
We focused on a small number of points, and, in order to guarantee observable effects, we enforced the best possible conditions for each visual variable to create distinct groups.
Other possible scenarios include a wider range of values as initial and final states (\eg, shades of gray instead of white or black), making the perceptual identification of groups more difficult.

To provide complementary findings applicable to more realistic data visualization settings with a larger number of visual objects, we also report on a follow-up study assessing the LCF for two types of trend visualizations: an animated scatterplot inspired by Gapminder,\footnote{\url{http://www.gapminder.org/}} as well as a dynamic thematic map of election data.

The focus of this study was on obtaining nuanced qualitative insight into more complicated use cases of the notion of common fate, to further our understanding of what influences grouping in a dynamic visualization.
Thus, we limit this follow-up experiment to the dynamic variants of the three visual variables: \DP, \DS, and \DL. 

In both visualizations, the magnitude of the change in the dynamic variables was mapped to the change in the underlying data variables.
Color scales used linear interpolation in the L*a*b* color space.
Animated transitions lasted 2 seconds and used linear interpolation.
Participants could replay the animation using a 'replay' button.
They entered written explanations for each question, but were also encouraged to think aloud, and to elaborate verbally on their written answers. 

\begin{figure*}[htb]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/follow-up-3}
  \vspace{-6mm}
  \caption{Grouping strength ranking results (numerical answers to Q3$^4$) for the three dynamic variables (\DP, \DS, and \DL) in the context of a Gapminder-like animated scatterplot visualization (left) and an animated thematic map of U.S.\ Presidential election data (right).}
  \label{fig:follow-up-3}
\end{figure*}

\subsection{Gapminder-like Animated Scatterplot}

In the animated scatterplot, each bubble represents a country and encodes four data dimensions: life expectancy, fertility rate, child mortality, and income (Figure~\ref{fig:follow-up-3}, left)~\cite{GapminderData:19}. 

In this condition, we presented participants with three different configurations of the scatterplot that we generated by varying the visual encoding of the four data dimensions.
% (Table~\ref{tab:gapminder-design}).
Life expectancy was always assigned to vertical position.
The other variables were each assigned to horizontal position, size, and luminance exactly once.
Apparatus is available at: \url{http://tiny.cc/gapminder_plot}

During each animated transition, all three visual variables (i.e.\ position, size, and luminance) change simultaneously to portray the change in the underlying data between 1960 and 2014 (linearly interpolating between the two years).
The visualization viewport was 600$\times$600 pixels, the radii of points varied between (4px, 14px), and luminance varied between (0.33, 1.00) since occlusion made distinguishing countries difficult when using pure black.

\subsection{Election Data Bubble Map}

In the map visualization (Figure~\ref{fig:follow-up-3}, right), an animated bubble is displayed on top of each state to represent two data dimensions: change in voter turnout~\cite{VoterTurnout12, VoterTurnout16} and Democratic vote share from 2012 to 2016~\cite{VoteShare12, VoteShare16}. 
All points started out with an identical color and radius to minimize the influence of the initial state. 
 
The study involved four different configurations of the map visualization that we generated by varying both the visual encoding of the two data dimensions and the section of the map that was displayed. Every participant saw the same four map sections, which each showed roughly one quarter of the U.S.\ (with some overlap) to reduce training effects between trials.
The two data dimensions were mapped to one of \DL or \DP in each trial.
Hence, the four configurations presented the combination of two different instances of visual encoding and four different map sections.
The viewport size was 800$\times$400 pixels, the radii of points varied between (4px, 14px), and luminance varied between (0.0, 1.0).
Apparatus is available at: \url{http://tiny.cc/election_map}

\subsection{Method}

We recruited 10 participants ($M_{age} = 24$, 4 female) using in-course announcements and university message boards.
Compensation was \$10 or course credit, and the experiment lasted 45--60 minutes.

The order of the two visualization conditions was counterbalanced between participants.
Participants answered all questions for every trial in each of the two conditions (total number of questions was 21):

\begin{enumerate}[nosep]
    \item[Q1.] What patterns do you see in the visualization?
    Describe (at least) 2--3 groups of points that behave in the same way.

    \item[Q2.] Which [country/state] is closest in behavior to the highlighted [country/state]?
    
    \item[Q3.] Which dynamic variable(s) create the most visible patterns?
\end{enumerate}

The experiment was audio recorded.
The participants were instructed to give written explanations for each of their answers, and were encouraged to give verbal details, so as to obtain rich qualitative feedback on their analytic process. 

\subsection{Results}

Results were based on a holistic analysis of participants' input, including written answers to the experimental trials, transcriptions of think-aloud comments, and answers to the follow-up survey questions.
The author who conducted the experiment developed a list of top-down themes that were used to analyze the data.

Overall, all participants successfully identified patterns using all three dynamic variables in response to Q1; \eg, \quote{small group of points moving horizontally... while also getting darker, but no significant change in size (P8)}, \quote{one set of points increase in size, another (possible overlapping) set go black (P6)}. 

In their answers participants also showed that they could effectively map dynamic changes in the visual variables to meaningful trends in the underlying data; \eg, \quote{points on the right got darker, while on average also increasing in size slightly.
This indicates that there was a negative change in Dem.\ vote share, with a small increase in voter turnout. (P8)}; \quote{Life expectancy for richer people gets higher (P7)}.
Overall, participants tended to reason in the data space for the pattern identification task (Q1), while they combined both data and visual space reasoning for the closest behavior task (Q2).

Most of the participants successfully performed conjunction search in response to Q2, by finding data points that changed similarly in all dynamic variables simultaneously. However, some others used only one or two visual variables out of three in the Gapminder example: \eg, P3 used only position and P5 used only two variables at a time (size and luminance or size and position).

Participants made semantically meaningful choices using the three dynamic variables with no access to information about the identity of the countries (\eg, Qatar was most often identified as closest in behavior to Kuwait while Thailand and Brazil were most commonly identified as similar to Vietnam).

\subsubsection{Relative Strength of Dynamic Variables}

Numerical answers to Q3\footnote{P5's answers for the map condition were reversed because her written justification made clear that she had inverted the scale.
P4's answers were excluded because he did not assign unique ranks to the dynamic variables.} (Figure~\ref{fig:follow-up-3}) provide a ranking that can be compared with the results of our crowdsourced study. 

In the Gapminder condition, \DP was overwhelmingly ranked as the strongest variable.
\DS appeared to be the next strongest, and was ranked first or second twice as often as \DL.
This deviates slightly from the first study, where \DP was only marginally stronger than \DS.

In the map condition, however, while \DL was ranked as the strongest variable slightly more often than \DS, there was no clear overall trend.
Participants commented that it was difficult to rank these variables, \eg, \quote{Between color and size, both seem equally prominent} (P5).
This again differs from past results, where \DS dominated \DL.

Differences in the underlying data caused rankings to vary between trials for the same participant, with only two participants assigning the same ranks to \DP and \DS for all four maps, and only one participant assigning completely consistent ranks in the Gapminder condition. 

\subsubsection{Dynamic Behavior}

Participants used both the dynamic behavior of the points and their initial and final states when identifying trends; \eg, P7 felt two countries were close in behavior \quote{because position-wise they're converging to the same place and... color-wise they're also doing same.} 
P9 focused on dynamic behavior; i.e., \quote{they didn't start... similar to each other, but their rapid growth was similar.}
When describing similarities in dynamic behavior, participants commented mostly on direction and magnitude of the change: \quote{It's moving the same way, moving in the same direction at nearly the same speed} (P6).
The perceived synchrony of change also seemed an important criteria for some participants when comparing dynamic behaviors: \quote{they changed almost at the same time... the brightness are getting darker, going to the same direction at the same time} (P5).

\subsubsection{Proximity}

Proximity was mentioned several times as an important cue for group formation.
Though our definition of common-fate similarity in \S~\hyperref[sec:similarity]{\ref{sec:similarity}} is independent of proximity (\SP-similarity), participants reported that it was easier to group data points together using one of the dynamic variables if they were close together; \eg, \quote{They are also close to each other, so it was easy to detect them} (P2), \quote{I guess I have greater confidence too, when it's closer} (P10).
In addition, when answering Q2, P4 reported focusing on countries near the target in the Gapminder condition, and P5 used proximity to the target to break ties between otherwise similar candidates in the map condition.
While the first experiment showed that \DP and \DS have stronger mean grouping strengths than \SP, these observations suggest that \SP-similarity could play a mediating role in the perception of all three dynamic variables.

While close distances seemed to facilitate comparison and group identification for some participants, sparsity also played an important role in detecting dynamic behaviors: \quote{This one is more noticeable than other circles because it's isolated} (P2); \quote{Position is very obvious. The circles are becoming extremely sparse!} (P7).

\subsubsection{Cardinality}

Several participants noted that the number of points that underwent a certain dynamic change increased the visibility of the patterns variable produced.
\quote{Brightness was... strongest because there were three points that changed in brightness dramatically while only one point changed in size} (P8), and \quote{The size was the strongest due to the larger amount of circles in this cluster} (P9).
On the other hand, a few participants felt that a small number of outliers that changed significantly in one dynamic variable could influence them to find the rest of the changes in that variable greater as well: \quote{those circles that move quickly, that kind of biases my mind} (P2), \quote{The white circle on the upper right catches my attention more than any other circles, so I tend to think the size is more noticeable} (P2).
Still, participants were also able to detect patterns involving a small number of data points: \quote{most countries decrease in fertility rate; a couple stay the same} (P1), \quote{Only a few circles both change income and life expectancy} (P2), and \quote{there is a group of 2 or 3 points which started in the bottom left and moved vertically upwards while slightly decreasing in size} (P8).

\subsubsection{Interactions Between Dynamic Variables}

One participant felt that because \DP drew his attention, he was more likely to notice changes in \DS in the vicinity: \quote{my eyes keep following that trend...the trend of position which correlates to stronger size changes (P10)}.
Position was also sometimes perceived as interfering with the other two variables: \quote{the color and the size...[are] so hard to see when there's so much stuff and it's moving so fast (P1)} .

%\jacob{find these quote - another participant felt that the change in size made the change in color hard to see}. 
%--Other relevant quotes:
%-------[Gapminder]
%-P8: "there isnt much changing in size in this visualization so size is ranked the weakest. Since points are still quite large when changing brightness, brightness is ranked second."
%-P8: i ranked brightness as the weakest since the points change in brightness after they had decreased in size which made it difficult to see as much as the change in size itself.
%-P10:  My vision seems to follow the trend of position which also correlates to stronger size changes
%-P10 (ranked DS as 3): Size: Most size changing here is happening in the part of the graph where little position change is occurring - I'm not as drawn to those changes.
%P10 (ranked DL as 2): Brightness: seems like many points start fairly bright and get darker. Also following position trend.
%P10: Color again was a bit less important partially due to occlusion.

%--------[Map]--------
%P1: (DL>DS) "the change in shade seems more dramatic. there is a group of white surrounded by others that seem to get darker making the white more pronounced"
%P8: DL>DS) "in addition, the points that changed in size the most were also the points that changed in brightness the most which made it less apparent."

%\begin{figure}[htb]
%  \centering
%  \includegraphics[width=0.95\linewidth]{figures/follow-up-results.pdf}
%  \caption{Results for ranking question.}
%  \label{fig:ranking_results}
%\end{figure} 
